Maximizing NFT Incentives: References Make You Rich

In this paper, we study how to optimize existing Non-Fungible Token (NFT) incentives. Upon exploring a large number of NFT-related standards and real-world projects, we come across an unexpected finding. That is, the current NFT incentive mechanisms, often organized in an isolated and one-time-use fashion, tend to overlook their potential for scalable organizational structures. We propose, analyze, and implement a novel reference incentive model, which is inherently structured as a Directed Acyclic Graph (DAG)-based NFT network. This model aims to maximize connections (or references) between NFTs, enabling each isolated NFT to expand its network and accumulate rewards derived from subsequent or subscribed ones. We conduct both theoretical and practical analyses of the model, demonstrating its optimal utility.

==> sub-sections/sub-ref.tex <==
\section{Preliminaries}\label{sec-preli}

\subsection{NFT}



\subsection{Building rNFT Network}


\subsection{Stackelberg Game}



\begin{comment}
    



\section{Overview of DAG-DSPs}\label{sec-system-model}
{

\subsection{System Components}

\subsection{System Workflow}


\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figures/architecture.pdf}
    \caption{System Architecture. \textcolor{violet}{ Describe the platform with a system figure.
The system introduced in this paper do not have to be in a exactly the same form as the MVP you are developing. The blockchain in the DAG-DSP system will barely be abstracted as a decentralized blockchain platform where NFT is enabled. The system will be separated into two layers:  The DSP where the frontend/backend/storage is located. The actual models and datasets are expected to be used, shared, and manipulated on this platform. At the same time, when a sharing operation of a model/dataset (named resources) is being requested and released on the DSP, an rNFT associated with this resource, is added to a DAG that is maintained by the second layer where the reference relationships across different resources will be marked and recorded. The incentive will barely be based on this relationship in the DAG and does not need to go through the first layer. Let the first layer focus on the business, while the second focuses on the incentive.}
 }
    \label{fig:enter-label}
\end{figure}
%\color{violet}@Lam: I have completed the system architecture, could you take a look?
%Describe the platform with a system figure.
%The system introduced in this paper do not have to be in a exactly the same form as the MVP you are developing. The blockchain in the DAG-DSP system will barely be abstracted as a decentralized blockchain platform where NFT is enabled. The system will be separated into two layers:

%\begin{itemize}
%    \item The DSP where the frontend/backend/storage is located. The actual models and datasets are expected to be used, shared, and manipulated on this platform.
%    \item At the same time, when a sharing operation of a model/dataset (named resources) is being requested and released on the DSP, an rNFT associated with this resource, is added to a DAG that is maintained by the second layer where the reference relationships across different resources will be marked and recorded. The incentive will barely be based on this relationship in the DAG and does not need to go through the first layer. Let the first layer focus on the business, while the second focuses on the incentive.
%\end{itemize}

}
\end{comment}
